Frequency analysis and filter design for directed graphs with polar decomposition

In this study, we challenge the traditional approach of frequency analysis on directed graphs, which typically relies on a single measure of signal variation such as total variation. We argue that the inherent directionality in directed graphs necessitates a multifaceted analytical approach that incorporates multiple signal variations definitions. Our methodology leverages the polar decomposition to define two distinct variations, each associated with different matrices derived from this decomposition. This approach provides a novel interpretation in the node domain and reveals aspects of graph signals that may be overlooked with a singular measure of variation. Additionally, we develop graph filters specifically designed to smooth graph signals in accordance with our proposed variations. These filters allow for bypassing costly filtering operations associated with the original graph through effective cascading. We demonstrate the efficacy of our methodology using an M-block cyclic graph example, validating our claims and showcasing the advantages of our multifaceted approach in analyzing signals on directed graphs.

==> other/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/polar_decomposition.tex <==
\section{Polar decomposition and variation}

%\subsection{Preliminaries}



%\section{Polar Decomposition Interpretation}

\subsection{Polar Decomposition}



%Mhaskar \cite{MHASKAR2018611} proposed the use of the left polar decomposition (LPD), obtained from the singular value decomposition (SVD), for developing a harmonic analysis framework for digraphs, with a frequency ordering defined with respect to the singular values of the  adjacency matrix $\Am$. 
%The use of the polar decomposition is key to our multiple GFT constructions because  any arbitrary $\Am$ can be factored into interpretable matrix factors.
%

Given an arbitrary real adjacency matrix $\Am$, its singular value decomposition (SVD) is given by $\Am = \Um\Sigmam\Vm\tran$, where $\Um$ and $\Vm$ are the unitary matrices of right and left singular vectors, 
respectively, and $\Sigmam$ is the diagonal matrix of singular values.  
Then, the LPD is given by $\Am = \Pm\Qm$, where $\Pm$ is a positive semi-definite (PSD) Hermitian matrix and $\Qm$ is a unitary matrix, while  
the right polar decomposition (RPD) is given by $\Am = \Qm\Fm$, where $\Fm$ is a PSD Hermitian matrix and $\Qm$ is the same as in the LPD. 
Both polar decompositions can be derived  from the SVD as:  
%The equivalence between the polar decomposition and the SVD can be shown through 
% \begin{equation}
\begin{align}
    \Am = \Um\Sigmam\Vm\tran &= \Um\Sigmam(\Um\tran\Um)\Vm\tran = (\Um\Sigmam\Um\tran)(\Um\Vm\tran) = \Pm\Qm\\
    &=\Um(\Vm\tran\Vm)\Sigmam\Vm\tran = (\Um\Vm\tran)(\Vm\Sigmam\Vm\tran) = \Qm\Fm,
\end{align}
% \end{equation}
% \begin{equation}
% \Am = \Um\Sigmam\Vm\tran = \Um(\Vm\tran\Vm)\Sigmam\Vm\tran = (\Um\Vm\tran)(\Vm\Sigmam\Vm\tran) = \Qm\Fm,
% \end{equation}
where $\Qm=\Um\Vm\tran$, $\Pm=\Um\Sigmam\Um\tran$, and $\Fm=\Vm\Sigmam\Vm\tran$.




\subsection{Symmetrization-based variation analysis}
The clear node-domain interpretations  of the symmetrizations with respect to the original adjacency $\Am$ lead to several distinct variation modes on $\Am$. 

Quantifying the smoothness of signals on $\Bm_{\text{in}}$ and $\Cm_{\text{out}}$ using $\xv\tran\Bm_{\text{in}}\xv$ and $\xv\tran\Cm_{\text{out}}\xv$, respectively, leads to a measure of signal smoothness with respect to indirect node connections on $\Am$. 
Note that the variation $\xv\tran\Bm_{\text{in}}\xv$
% \begin{equation}
% \xv\tran\Bm_{\text{in}}\xv = \sum_ix(i)\sum_{j\in N_{\Bm}(i)}b_{ij}x(j) = 2\sum_{i\sim j}b_{ij}x(i)x(j)
% \end{equation}
is maximized for the eigenvector $\uv_{b,1}$ corresponding to the largest eigenvalue $\lambda_{b,1}$ of $\Bm_\text{in}$. 
The eigenvector $\uv_{b,1}$ has all non-negative entries (if $\Bm_{\text{in}}$ is disconnected, there will be multiple eigenvectors corresponding to the largest eigenvalue $\lambda_{b,1}$, with strictly positive values corresponding to each disconnected component in $\Bm_{\text{in}}$). Therefore, the smoothest eigenvector $\uv_{b,1}$ for $\Bm_{\text{in}}$ is a signal on $\Am$ that has low variation over nodes that share common in-links (Fig.~\ref{fig:symm_examples}). The same reasoning shows that the ``highest frequency" eigenvector $\uv_{b,N}$, corresponding to the smallest $\lambda_{b,N}$, is a graph signal with high variation over nodes that share common in-links. The full set of eigenvectors of $\Bm_{\text{in}}$ forms an orthonormal basis that captures different levels of signal variation over nodes that share common in-links. 
Similarly, the eigenvectors of $\Cm_{\text{out}}=\Am\tran\Am$ form an  orthonormal basis that captures different levels of signal variation over nodes that share common out-links (Fig.~\ref{fig:symm_examples}).
We next use the interpretation of variations corresponding to symmetrizations to describe the properties of the GFT bases obtained from the LPD and RPD factors.

    \begin{figure}[t]
	\centering
	\includegraphics[width=.7\linewidth]{figures/freq_support_separable_filt.pdf}
	\caption{To illustrate the separable node-domain interpretation of the general single-mode frequency ordering based on the adjacency TV ordering \cite{Sandryhaila_2013_2}, the eigenvalues $\lambda_a$ of a $N=100$ directed torus graph (normal $\Am$) are plotted. As $\Am$ is normal, the direct relations $|\lambda_a| = \lambda_p$ and $e^{i\omega_a} = \lambda_q$ provide a clear node-domain interpretation of the $\lambda_a$ locations on the unit disc. Colors indicate distance of each $\lambda_a$ to $|\lambda_{a}|_\text{max}$, therefore, $|\lambda_a - 2|$. The two eigenvalues circled in red correspond to eigenvectors of $\Am$ with very similar variation measures (2.62 and 2.76) with respect to the total variation definition in \cite{Sandryhaila_2013_2}. However it is clear that both eigenvectors have very different variation in terms of the spectra of $\Pm$ and $\Qm$ (i.e. very different indirect variation and inflow variation).}
	\label{fig:freq_support}
    \end{figure}

\subsection{Polar Decomposition GFT Basis Definitions}
The eigendecompositions of the three factors ($\Pm$, $\Fm$, and $\Qm$) from the LPD ($\Am=\Pm\Qm$) and RPD ($\Am=\Qm\Fm$) provide three distinct bases.
We first state the  definitions of these bases and their respective variation measures, before providing a more in-depth analysis of their node-domain variation interpretations in the subsequent section. 

\textbf{Common In-Link Basis}: Let $\Pm=\Um_p\Lam_p\Um_p\tran$, where the columns of $\Um_p$ consist of the orthonormal eigenvectors of $\Pm$, and $\Lam_p$ is the diagonal matrix of non-negative eigenvalues. The set of eigenvectors $\Um_p$ form an orthonormal GFT basis capturing variation over nodes with \textbf{common in-links} on $\Am$. The eigenvector variation ordering is determined by $\uv_p\tran\Pm\uv_p$.

\textbf{Common Out-Link Basis}: Let $\Fm=\Um_f\Lam_f\Um_f\tran$, where the columns of $\Um_f$ consist of the orthonormal eigenvectors of $\Fm$, and $\Lam_f$ is the diagonal matrix of non-negative eigenvalues. The set of eigenvectors $\Um_f$ form an orthonormal GFT basis capturing variation over nodes with \textbf{common out-links} on $\Am$. The eigenvector variation ordering is determined by $\uv_f\tran\Fm\uv_f$.

\textbf{In-Flow Basis}: Let $\Qm=\Um_q\Lam_q\Um_q^H$, where the columns of $\Um_q$ consist of the unitary eigenvectors of $\Qm$, and $\Lam_q$ is the diagonal matrix of unit modulus eigenvalues. The set of eigenvectors $\Um_q$ form a unitary GFT basis capturing variation over nodes connected by \textbf{in-flow links} on $\Am$. 
Given that all eigenvalues reside on the unit circle, the eigenvector $\uv_{q,i}$ corresponds to the angular frequency $\omega_{q,i}$ of the associated eigenvalue $\lambda_{q,i}=e^{j\omega_{q,i}}$ \cite{unitaryshift}.


\subsection{Variation Interpretations of the Bases}

We propose to use the three GFTs ($\Um_p, \Um_f, \Um_q$)  in parallel to  analyze multiple types of signal variations  on arbitrary digraphs. 

The bases $\Um_p$ and $\Um_f$ both capture what we refer to as \textbf{indirect variation}. 
Note that $\Pm=\sqrt{\Bm_{\text{in}}} = \sqrt{\Am\Am\tran}$ and $\Fm=\sqrt{\Cm_{\text{out}}}=\sqrt{\Am\tran\Am}$. 
As $\Bm_{\text{in}}$ and $\Cm_{\text{out}}$ are symmetric matrices and are therefore orthogonally diagonalizable, $\Bm_{\text{in}}$ and $\Cm_{\text{out}}$ share the same eigenvectors as $\Pm$ and $\Fm$, respectively. 
In addition, $\Pm$ and $\Fm$ share the same eigenvalues, which are the square roots of the eigenvalues of $\Bm_{\text{in}}$ and $\Cm_{\text{out}}$. 
Both factors can be written as $\Pm = \Um_b\sqrt{\Lam_b}\Um_b\tran$ and $\Fm = \Um_c\sqrt{\Lam_c}\Um_c\tran$ with $\Lam_b=\Lam_c$. Since $\Pm$ and $\Fm$ share the same eigenvectors as $\Bm_{\text{in}}$ and $\Cm_{\text{out}}$ with the same eigenvalue ordering (as the square root preserves their ordering), it is clear that $\Pm$ and $\Fm$ capture the same signal variation information with respect to the original $\Am$ as $\Bm_{\text{in}}$ and $\Cm_{\text{out}}$, respectively. 
Therefore, the eigenvectors of $\Pm$ capture different levels of signal variation over nodes that share common in-links on $\Am$, and the eigenvectors of $\Fm$ capture different levels of signal variation over nodes that share common out-links on $\Am$.

The basis from $\Um_q$ captures what we refer to as \textbf{in-flow variation}. 
% Q is simlar to A
A key property of $\Qm$ is that it is the closest unitary matrix to $\Am$ with respect to any unitarily invariant norm \cite{graph_mining}. 
This implies that $\Qm$ is the closest matrix to $\Am$ for which a graph multiplication is lossless ( $||\xv||_2=||\Qm\xv||_2$). 
Thus, the ``graph shift''  operation $\Qm\xv$ can be reversed through multiplication with $\Qm\tran$.
% If the graph is strongly connected, the graph that supports Q as the adjacency matrix has Hamiltonian cycle
Also, if a graph is strongly connected that supports a unitary matrix as adjacency matrix, the graph is Hamiltonian, meaning that it has a cycle that contains all the vertices exactly once~\cite{severini2003digraph}.
Therefore, we can view $\Qm$ as an alternative adjacency matrix with a direct relation to $\Am$ adding edges to have Hamilton cycles.
In Fig.~\ref{fig:symm_examples}, for example, the graph that supports $\Qm$ as an adjacency matrix has five additional edges (arrows with red color) compared to the original graph allowing the new graph to have Hamiltonian cycles (e.g., 0-2-4-6-1-3-5-7-0).
We then define our variation metric, as previously stated.
% In addition, $\Qm\Qm\tran=\Qm\tran\Qm=\Id$. 
% Similar to what we did with $\Pm$ and $\Fm$,  
%as alternative adjacency matrices with clear node-domain interpretations with respect to $\Am$, 


% Therefore $\Qm$ is the closest unitary matrix to $\Am$ for which the \textbf{indirect variation} modes are trivial. For this reason, we claim that the eigenvectors of $\Qm$ capture the complementary variation information to the indirect variation captured by $\Pm$ and $\Fm$.

If $\Am$ is normal, i.e., such that $\Am\Am\tran = \Am\tran\Am$, there is a direct correspondence between the magnitude and phase components of its eigenvalues $\lambda_a = |\lambda_{a}|e^{i\omega_{a}}$, and the eigenvalues of $\Pm$, $\Fm$, and $\Qm$ (for normal $\Am$, $\Pm=\Fm$). The magnitude $|\lambda_a|$ corresponds to an eigenvalue $\lambda_p$ of $\Pm$ with $\lambda_p=|\lambda_a|$. The phase $e^{i\omega_{a}}$ corresponds to an eigenvalue $\lambda_q$ of $\Qm$ with $\lambda_q=e^{i\omega_{a}}$.
Therefore, $|\lambda_{a}|$ indicates the smoothness of a signal on $\Am$ over nodes that share common-in/out links, and $e^{i\omega_{a}}$ indicates the smoothness of a signal over the in-flow connections of a graph Fig.~\ref{fig:freq_support}. 
This direct relation between the eigenvalues of $\Am$ and the spectrum of $\Pm$, $\Fm$, and $\Qm$ that holds for normal matrices provides a separable interpretation of the magnitude response of polynomial filters of $\Am$. 
A polynomial filter of a normal $\Am$, $p(\Am)$, assigns a specific gain with respect to each $\lambda_a$, therefore, one could implement a filtering operation in the frequency domain of $\Am$ by cascading filtering operations in the spectral domain of $\Pm$ and $\Qm$. 
Note that, as show by the circled points  Fig.~\ref{fig:freq_support}, two eigenvectors with very similar variation with respect to $\Am$, i.e., similar $||\lambda_{a,\max}|-\lambda_a|$ may have very different in-flow  ($\lambda_q$) and indirect   ($\lambda_p$) variations. This will be further shown experimentally in the case study of Section~\ref{sec:m-block}. 
% , since a function of  $\lambda_a$  can be represented in terms of functions of $|\lambda_a|$ and $e^{i\omega_{a,j}}$. 

However, for non-normal matrices, the lack of a direct correspondence between $\lambda_a$, $\lambda_p$, and $\lambda_q$ implies that a filter based on $\Am$ cannot be separated in terms of filters that are polynomials of $\Pm$ and $\Qm$. 
%
%the parallel GFT based analysis to result in a function of the spectra' of $\Pm$ and $\Qm$ that cannot be directly replicated by a function of $\Am$.
%
Even with this lack of correspondence for non-normal $\Am$, indirect variation and in-flow variation together allow us to interpret the eigenvalues of $\Am$ \cite{Sandryhaila_2013_2}. 
While the frequency ordering corresponding to complex $\lambda_a$ is not unique, the frequency orderings corresponding to $\lambda_p$ and $\lambda_q$ are both unique.
